The miniJPAS survey: a preview of the Universe in 56 colours

The Javalambre-Physics of the Accelerating Universe Astrophysical Survey (J-PAS) will soon start to scan thousands of square degrees of the northern extragalactic sky with a unique set of $56$ optical filters from a dedicated $2.55$m telescope, JST, at the Javalambre Astrophysical Observatory. Before the arrival of the final instrument (a 1.2 Gpixels, 4.2deg$^2$ field-of-view camera), the JST was equipped with an interim camera (JPAS-Pathfinder), composed of one CCD with a 0.3deg$^2$ field-of-view and resolution of 0.23 arcsec pixel$^{-1}$. To demonstrate the scientific potential of J-PAS, with the JPAS-Pathfinder camera we carried out a survey on the AEGIS field (along the Extended Groth Strip), dubbed miniJPAS. We observed a total of $\sim 1$ deg$^2$, with the $56$ J-PAS filters, which include $54$ narrow band (NB, $\rm{FWHM} \sim 145$Angstrom) and two broader filters extending to the UV and the near-infrared, complemented by the $u,g,r,i$ SDSS broad band (BB) filters. In this paper we present the miniJPAS data set, the details of the catalogues and data access, and illustrate the scientific potential of our multi-band data. The data surpass the target depths originally planned for J-PAS, reaching $\rm{mag}_{\rm {AB}}$ between $\sim 22$ and $23.5$ for the NB filters and up to $24$ for the BB filters ($5\sigma$ in a $3$~arcsec aperture). The miniJPAS primary catalogue contains more than $64,000$ sources extracted in the $r$ detection band with forced photometry in all other bands. We estimate the catalogue to be complete up to $r=23.6$ for point-like sources and up to $r=22.7$ for extended sources. Photometric redshifts reach subpercent precision for all sources up to $r=22.5$, and a precision of $\sim 0.3$% for about half of the sample. (Abridged)

==> Mini_jpas_sections/205_pipeline_old.tex <==
\def\sext{\texttt{SExtractor}}


{\color{red} To be edited by Jesus. Note, the current text is a mix from the J-PLUS paper and the online documentation with some edits}

The \jp data, like all the scientific data produced by the OAJ, are
handled, processed, final coadded images construction and the
construction of the catalogues with the measurements of the objects
detected in the latter.

\subsection{Processing of single frames}

The detrending of the single frames follows the standard procedures of
bias subtraction, pre/overscan subtraction, trimming, flat field
correction, illumination correction and, if needed, fringing
corrections. More detailed information of how these steps have been
implemented for other OAJ surveys (ie. J-PLUS) can be found
in~\citet{cenarro2019}.

Now we will focus on few particular aspects that needed specific
treatment for \mjp\ data with respect to the of J-PLUS. The origin of
the need for these changes or specific implementation can be found on
the fact that Pathfinder camera wasn't designed specifically for the
JST and, as a result, we have to face several optical issues
(reflections, strong gradients, background patterns,...) that were
present in Pathfinder images. However, we don't expect this to be the
case for JPCam images since the design of this one was part of the
overall optical design of the system JPCam+JST.

The first issue that we detect on Pathfinder images was a strong
vignetting in the outer part of the CCD. The resulting images showed a
strong gradient of efficiency. To minimize the impact on the final
measurements, it was opted for trimming the images to an area in which
the efficiency would be enough large. The preliminary tests imposed a
reduction of the effective area of the CCD from 9216 $\times$ 9232
pixels to 7777 $\times$ 8473.

\textcolor{red}{(Jesús: Check whether this is also commented in the
  section about Pathfinder)}

The other important issue that was detected in Pathfinder images was
background patterns with strong gradients and changing in time scales
of few minutes. These patterns differed among group of filters due to
different origins. We were able to characterize at least two kind of
reflections for which we can guessed two different origins: a first
pattern with straight patterns most likely due to the optics of the
camera; and a second circular pattern affecting many of the reddest
filters whose origin most likely is due to the variation of the
central wavelength of the transmission curves of the filters
\textcolor{red}{(Jesús: Show figures?)}. In both cases, the net effect
is a irregular distribution of the sky light and this affect the
images in two ways: first, affecting the flat field images, producing
a spurious change of efficiency that needs to be corrected with the
illumination correction; and second, an irregular background pattern
that should be correctly subtracted to not affect the photometry of
the objects.

The illumination correction is part of OAJ standard reduction
procedure (\textcolor{red}{(Jesús: ask Héctor which paper cite for
  this)} and for this purpose, specific observations were planned
during \mjp\ observing campaigns. After constructing the master
illumination correction images (ICOR, hereafter), these were applied
to the images just after the flat field correction. Images corrected
by illumination correction show a background pattern not visible in
flat field corrected images. Although apparently in contrast with the
expectation for a ``correction'', this is indeed how it should
be\textcolor{red}{(Jesús:Add REF)}. The apparent removal of the
background pattern by the flat field is actually a consequence of the
same origin and both, flat field and background, follow the same 2D
pattern. However, the removal with the flat field is wrong and it is
not only wrongly ``flattening'' the background but also is affecting
the photometry of the objects. This last effect is the one corrected
by the illumination correction which is also recovering the original
background of the raw image. Nevertheless, considering that the
physical origin of this effect in flat field images and in the
scientific image, it is possible to compute a map of background with
the same 2D pattern of the ICOR but with the correct background level
of the scientific image. This was idea was tested and the resulting
images showed a flatter background and it was checked that the
photometry of the objects wasn't affect. Therefore, we introduce this
ICOR's related background subtraction just after the ICOR subtraction.

However, even after this background subtraction using the ICOR, still
remained in many single frames background patterns whose spatial
distribution made them difficult to be properly managed in a massive
automatic way during the source detection process, ie. with \sext. As
has been said above, these patterns have two main characteristics that
make this very difficult: presence of strong background gradients and
strong temporal variability of those patterns either in intensity of
spatial distribution.

Under the assumptions that these patterns are instrumental, and therefore
don't depend on the sky position (at least for enough close pointings),
and that they are stable in time scales of few minutes, we can
consider that images taken close in time (with the same filter)
present the same background pattern and, hence, a median combination
of scientific images with celestial objects in different positions
should keep the background pattern while removing the real
astrophysical objects. This is a procedure analogue to the
construction of master fringing images or superflat images, for this
reason we dubbed these background images as ``superbackground
images'' (SBGK, hereafter). 

However, the observational strategy of \mjp\ in which the single
exposures of the same pointing and same filter were taken with small
dithering and one after the other, introduced one problem and provided
an advantage. First, to not subtract light of real objects when
constructing the SBGK it is needed to avoid to have celestial objects
falling in the same parts of the images among the images combined to
construct the SBGK. Due to the temporal variation of the patterns
(with detected changes in scales of several minutes), it was not
possible to combine images of the same filter and different pointings
since they already showed changes in the background. Therefore, we
were left with the only possibility of having to use the images of the
same pointing and, due to the small dithering pattern, the chances of
having areas of the image covered by actual objects were high, in
particular for larger diffuse objects. To minimize this possibility,
before combining the images, the objects detected in a preliminary
reduction without SBKG correction were masked with masks a bit larger
than the actual detected size of the object to take into account
extended diffuse light. This masking procedure was fine-tune until it
was checked that there were no residuals of extended galaxies in the
SBGK (for bright saturated stars we allowed for light of their halos
to be in the SBKG). In the specific case of \mjp\ data, being a
cosmological field devoid of large galaxies (ie. galaxies occupying a large
area of the CCD), the possible oversubtraction of background due to
this procedure wasn't a big issue, although for the studies of faint
extended studies this has to be in mind.

In summary, the SBKG construction consisted, first, in identifying the
images to be combined. That was done taking advantage that exposures
of the same pointing and same filter were done consecutively and,
therefore, we could consider that in the interval between the first
and last exposure the background pattern was stable (although in few
cases we detected that this wasn't the case and some residuals were
left). Then, objects were masked and images median-combined. Finally,
the resulting image was smoothed using \sext\ and keeping the
background image that created. The last step was to subtract the SBKG
to the individual scientific frames.

In order to verify that the SBGK correction didn't affect the
photometry of the objects we simulate the construction of an ICOR (a
procedure that by construction shows changes in photometry of object
across the CCD) applying all the corrections to the images to be used
and the resulting map was compatible with no correction.

AS it was stated above, regarding J-PAS, since the optical design of
JPCam was done together with that of the JST, we expect to not suffer
this kind of background pattern or not in such strong degree. Besides,
a suitable observational strategy avoiding consecutive observations of
the same area of the sky with a small dithering pattern would help in
the construction of optimal superbackground images in which even large
diffuse light would be treated properly.

For filters redder than J0740, the presence of fringing makes
necessary a final step to remove that pattern. In this case, we follow
the standard implementation already in used for the J0861 filter of
J-PLUS. In contrast with the previous background issues, fringing
pattern is very stable across nights and we were able to construct
master fringing images using as many images taken with Pathfinder in
each of the filters. Unfortunately, for some filters there weren't so
many and in other cases the pattern was particularly string (special
mention here for the J1007 filter), and the result was a non-optimal
subtraction of the fringing pattern whose residuals are visible in the
final images. For these reason, we call the attention to the readers
when using or interpreting the results of the reddest filters.

One last step needed for the proper combination of the images is their
astrometric calibration. This is carried out again as a part of the
standard procedure for OAJ images using the software \texttt{Scamp}\citet{bertin2010scamp}
and the Gaia DR2\citet{gaia2018} as reference catalogue.






\subsection{Final coadded images}

Next, once the single frames were cleaned of instrumental trends, they
were combined with the
Astromatric\footnote{\url{https://www.astromatic.net}} software
\texttt{Swarp}\citep{bertin2010}. All the images were sampled to the
fiducial pixel size of the camera (ie. 0.227"/pixel), including all
the images of the narrow bands that were observed with a binning of
2$\times$2. We opted for keeping as close as possible the orientation
of the original frames instead of forcing to have the coadded images
oriented with North towards up (increasing Y axis) and East toward
left (decreasing X axis). In addition to the combined scientific
image, \texttt{Swarp} also constructs a normalized weight image that
keep track, for example, of areas were the number of combined images
is lower (for example in the edges due to the dithering pattern but
also in regions were spurious detection were previously masked in one
or more single frames). Therefore, the weight image can be considered
as a map of the effective exposure time of the different parts of the
image and this is taken into account, for example in the masking
process explained below.

The final stage consists in the elaboration of different types of
products extracted from the final coadded image to help in the proper
scientific exploitation of the original observations.

The main products are the photometric catalogues with the detections
and measurements for all the detected objects. In addition to it we
provide with some ancillary data that may help in the analysis or the
postprocessing of the data. In particular, we provide with detailed
models of the PSF across all the images and with masks that help to
identify problematic areas of the survey.

In the following sections we briefly explain how the main photometric
catalogues are constructed~\ref{sec:catalogues} and, then, how the
models of the PSF are constructed~\ref{sec:psf}, the construction of
masks of problematic areas~\ref{sec:masks}.

\subsection{Photometric catalogues\label{sec:catalogues}}

\textcolor{red}{(Jesús: I think that in this section should be everything
  related with how things are computed, e.g. construction of
  catalogues (source extraction, dual/single modes differences,...),
  while in the next section should be a description of 
  what it is produced emphasising those points prone to confusion)}

The detection of sources in the images is done with the widely used
software \sext\citep{bertin1996}. To cover as much as possible the
needs of the astronomical community we have run \sext\ in two
different complementary ways:
\begin{description}
\item[Dual-mode] To construct catalogues in which the photometry in
  the different bands for each object is done consistently, we have
  run \sext\ in the so called ``dual-mode''. In dual-mode, \sext\ is run
  first in a reference image for source detection and definition of
  position and sizes of the apertures and then is run in a target
  image in which the photometry is performed in the apertures defined
  by the reference image. In our case, we chose r band images as
  reference images for constructing the dual-mode catalogues.
\item[Single-mode] In the so called ``single-mode'' both the detection
  and the photometry are performed in a single image. This means that
  each image of each pointing and each band is treated completely
  independent. This has the advantage of detecting objects with no
  detection in the reference band (eg. faint object with strong
  emission lines out of the r band) with the drawback that the
  photometry in the different bands of each object can be done in
  slightly different positions producing inconsistent colours.
\end{description}

The detection parameters were set to particular values to increase
detectability (ie. increase completeness) while avoiding spuriours
detections (ie. increase of purity). Due to higher noise in all the
bands different to the r band, the detection threshold (in units of
the $\sigma$ of the background) for the generation of single-mode
catalogues were set to a higher value (\texttt{DETECT\_THRESH=2}) than
for the dual-mode catalogues~(\texttt{DETECT\_THRESH=0.9})\footnote{For
  completeness, this is the value of the other controlling the source
  detection: \texttt{DETECT\_MINAREA}=5.}.
  
  
  
  
  

\subsection{Photometry}

We provide different measurements of the flux of each individual
objects in order to cover as much as possible the necessity of the
astronomical community. Following, we provide a description of the
different types of photometric measurements that are provided in the
database.

First of all, we provide the photometry either in dual-mode and
single-mode: 
\begin{description}
\item[Dual-mode photometry] For mini-JPAS data, the dual mode
  catalogues are constructed using the r band images as detection
  image. Dual-mode catalogues ensure that, apart from the effect of
  variation of the PSF among images, the photometry in all the bands
  is performed in the same area for each object, producing consistent
  color measurements. Therefore, dual-mode catalogues are the suitable
  one for most of the astronomical analysis. However, ac couple fo
  things should be kept in mind to avoid confusion when using these
  dual-mode catalogues:
  \begin{itemize}
  \item Although the r band, being the deeper one, has been chosen as
    the detection band, for faint objects with particular SEDs, it
    can happen that the object is not detected in r band while it can
    be detected in other band. In these cases, single-mode catalogues
    are more suitable.
  \item Since the apertures in all the bands are defined in the r
    band, for very faint object with fluxes within the noise in bands
    different than the detection one, it is possible to measure
    negative fluxes. This is not a problem and is consistent with the
    fact of measuring within the noise.
  \end{itemize}

% Leave this better for the Data Products section since we need to
% introduce the photometric calibration first.
%  This photometry is stored in the database in tables with the tag
%  \texttt{Dual} in their names, e.g. \texttt{MagABDualObj}.
\item[Single-mode photometry] In this case, the detection and
  photometry in each band is done independently and as such, in the
  database the measurements on different bands are treated
  independently leaving the freedom to the user to decide the way to
  identify the measurements of a given object.

% DITTO
%  This photometry is stored in the database in tables with the tag
% \texttt{Single} in their names, e.g. \texttt{MagABSingleObj}.
\end{description}

\textcolor{red}{(Jesús: I think this part is better here while I
  understand that the detailed description of the magnitudes is better
  to be put in the section of data products)}.

% At a final stage, the pipeline combines the processed images from the same sky
% area to provide a deeper, photometric calibrated image for each filter. The
% pipeline makes use of the packages {\tt Scamp} \citep{2006ASPC..351..112B} and
% {\tt Swarp} \citep{2002ASPC..281..228B} to perform the astrometric calibration
% and image coadding. The combined images for a given tile in the whole set of
% filters constitute a datacube. {\tt SExtractor} source catalogues are extracted
% from the final tiles and datacubes and are stored in an internal database
% system. Two kind of catalogues are produced. In the first one single-mode
% catalogue, the source
% detection and segmentation are done independently for the combined images in
% each filter. In the second one, the detection and aperture definition is done in
% the $r$ band, which is used as a reference image. More information on the
% ``single-'' and ``dual-mode'' catalgues are provided in Section
% \ref{sec:data_products}.  Prior to computing the final
% catalogues, the PSF of each filter image is homogenized to match the one of the
% $r$ filter, defined as reference filter in \jplus. This technique was already
% used to produce the photometric catalogues for the
% ALHAMBRA survey \citep{2014MNRAS.441.2891M}, and more information are provided
% below. 


The final step for the photometric catalogues is the photometric
calibration of the fluxes. 

%\item{{\bf Photometric calibration}}
The photometric calibration of the mini-JPAS observations was adapted from the methodology presented in \citep{clsj19jpluscal}, developed to provide the calibration of the J-PLUS project. We applied the following steps:

\begin{enumerate}
\item Definition of a high-quality sample of stars for calibration. We selected those mini-JPAS + {\it Gaia} sources with $S/N > 10$ in all the photometric bands and with $S/N > 3$ in {\it Gaia} parallax. We constructed the dust de-reddened absolute $G$ magnitude vs. $G_{BP} - G_{RP}$ colour using the information from the 3D dust maps in \citep{green+18}, and selected those sources belonging to the main sequence. This provides 334 calibration stars.

\item Calibration of the $gri$ broad-bands to the Pan-STARRS photometric solution. We compare the 6$\prime\prime$ aperture instrumental magnitudes corrected by aperture effects in mini-JPAS with the PSF magnitudes in Pan-STARRS. This provide the zero points of the $gri$ broad bands. We computed also the zero points by comparison with J-PLUS photometry, obtaining differences below 5 mmag.

\item Homogenization of the narrow bands with the stellar locus. We compute the dust de-reddened $(\mathcal{X}_{\rm ins}-r)_0$ vs. $(g-i)_0$ colour-colour magnitude of the calibration stars and computed the offsets that provides a consistent stellar locus among the pointings. This provided a homogeneous instrumental photometry in mini-JPAS.

\item Absolute colour calibration. The last step is to translate the instrumental magnitudes on top of the atmosphere. This step was done in J-PLUS with the white dwarf (WD) locus, but there is no high-quality WD in the mini-JPAS area. We therefore used BOSS stellar spectra as reference to provide the absolute calibration of mini-JPAS colours. After a visual inspection of the available BOSS spectra, we ended with 40 stars. We compared the synthetic $(\mathcal{X}-r)$ colours from BOSS spectra with the instrumental magnitudes from mini-JPAS to obtain one offset per passband but $r$, that is used as reference and anchored to the Pan-STARRS calibration.

\item The BOSS spectra do not cover the $uJAVA$ and $uJPAS$ filters. In this case, we obtained the colour offset by direct comparison with J-PLUS photometry.

\end{enumerate}

Summarising, the flux calibration of mini-JPAS photometry is referred to the Pan-STARRS $r$ band and the colours are anchored to the BOSS spectra.

We estimate the zero points also by direct comparison with J-PLUS photometry in those shared or similar passbands. Such comparison provides consistent zero points at the 4\% level. Thus, we conclude that the current photometric calibration has an absolute error of 0.04 mag. We expect to reach a 1-2\% accuracy in the J-PAS photometric calibration when $\sim500$ deg$^2$ are gathered. This will permit a consistent colour calibration with the WD locus and a robust estimation of the uncertainties thanks to a large number of overlapping areas with duplicated measurements of the same sources.




\subsection{PSF treatment} \label{sec:psf}

One of the challenges of large field surveys is to provide homogeneous photometry for a large number of objects. Each J-PAS pointing is composed by 60 coadded images from multiple exposures. Variations in the PSF from filter to filter will produce inhomogeneous photometry since the light coming from same areas of the sky will be redistributed differently in the final image depending on the filter used.

This discontinuous PSF variations can cause problems in the photometry
for objects with a quite different PSF between the tiles. The
homogenization process allows PSF-Matched aperture-corrected
photometry measurements more consistent at the expense of degrading
some images (see Section~\ref{sec:photometry}).  This method uses
PSFEx~\citep{bertin2011} to calculate a PSF homogenization kernel, to
convert variable instrumental PSFs to constant round Moffat profiles
for practical purposes. We need to take into account that the
homogenization process has consequences in the image noise and
generates variable noise correlations over the image pixels.  For that
reason, the algorithm recalculates the noise model of the images that
latter is used to compute photometric errors\citep{molino2014}.  We
  only apply the homogenization kernel to the corrected PSF apertures
  (\texttt{PSFCOR} and \texttt{WORST\_PSF}, see
  Section~\ref{sec:photometry}) in the dual-mode catalogs, for all
  other apertures no convolution takes place.

As product of the PSF analysis of the images, we provide for each
image not only the overall PSF model produced by PSFEx, but we have
also developed a service that generates on-demand an actual image of
the PSF model in any position of any image.


\subsection{Masks\label{sec:masks}}

After the construction of the final coadded image, the next step is
the construction of masks covering areas with known problems. These
masks help to identify doubtful objects (see Sect.\ref{sec:flags}) and
to remove complete problematic areas of the survey for particular
analysis like number counting.

Following we present a more detailed description of the three types of
masks that are generated:
\begin{description}
\item[\textbf{Window frame mask}] Mark sources that are outside the window
  frame. This mask is determined from the tiling weight-map image, in
  order to homogenize the effective exposure times for the same coadd
  and masking regions where the normalized weight map values are less
  than 85\%. This value has been selected to be a compromise to
  maximize the valid observation area and minimize regions with less
  effective exposure time where, usually, a lower number of images
  have been combined. However, for each object we compute the value of
  the normalized weight map at its position, which is stored in the
  parameter \texttt{NORM\_WMAP\_VAL}. This parameter takes a value of
  1 in the area with highest effective exposure.
\item[\textbf{Mask of bright stars}] The mask of bright stars blocks out
  regions around bright stars found in the Bright Star
  Catalog\footnote{\url{https://heasarc.gsfc.nasa.gov/W3Browse/star-catalog/bsc5p.html}}
  and the Tycho-2 catalog\citep{hogg20000}. The radius of each masked
  region is a function of the magnitude of the star.
\item[\textbf{Mask of artefacts}] Due to light reflections in the
  telescope or its optical elements it is possible to see artefacts or
  other issues in the coadd images. Using algorithms of automatic
  detection of artefacts or patterns in catalogues, these problems can
  be detected, analyzed and masked. in addition, if some artefact has
  not been detected automatically, we have developed a tool to
  manually mask it.
\end{description}

From the practical point of view, all the masks are stored as files
with the MANGLE 
software\footnote{\url{https://space.mit.edu/~molly/mangle/}}\citep{swanson2008}.
%To \mangle, a mask is an arbitrary union of arbitrarily weighted
%angular regions bounded by arbitrary numbers of edges.

We provide the masks for each tile or coadded image as well as a
combined mask of the whole \mjp\ footprint\footnote{The masks are
  available for download in the ``Image Search'' service of the
  Catalogues Portal.}



